Probabilistic Matrix Factorization for Automated Machine Learning

In order to achieve state-of-the-art performance, modern machine learning techniques require careful data pre-processing and hyperparameter tuning. Moreover, given the ever increasing number of machine learning models being developed, model selection is becoming increasingly important. Automating the selection and tuning of machine learning pipelines consisting of data pre-processing methods and machine learning models, has long been one of the goals of the machine learning community. In this paper, we tackle this meta-learning task by combining ideas from collaborative filtering and Bayesian optimization. Using probabilistic matrix factorization techniques and acquisition functions from Bayesian optimization, we exploit experiments performed in hundreds of different datasets to guide the exploration of the space of possible pipelines. In our experiments, we show that our approach quickly identifies high-performing pipelines across a wide range of datasets, significantly outperforming the current state-of-the-art.

==> extensions.tex <==
\section{Possible extensions}

\subsection{Predicting computational cost}
Some machine learning worflows are more computationally expensive to evaluate than others, so it would be desirable to be able to predict the running time of different workflows such that cheaper ones can be tried first (and more expensive ones can be tried only if they are really worth the time). Our prediction framework can be easily extended to this use case by simply collecting the running time statistics for $N$ models applied to $D$ datasets in a matrix $\mathbf{R} \in \reals^{N \times D}$ and pass it instead of $\data$ to the model described in section \ref{sec:main}. The predicted running time can then be integrated in the acquisition function by computing for instance an expected improvement per second, as suggested in \cite{snoek2012practical}.

\subsection{Adding metadata about the models and the datasets}
The model we described in section \ref{sec:main} learns correlations between different machine learning workflows induced by how correlated their performance is across the datasets in the training set. Often additional meta-data about the worflow and/or the model is available and can be easily incorporated in our model.

Examples of dataset metadata could be summary statistics such as: the number of samples, number of classes, number of features, etc. These meta features can be included by extending the covariance function described in section \ref{sec:main} to include a second covariance defined over the meta-features

\[
p(\data \given \latent, \btheta, \sigma, \metadata) = \mathcal{N}(\mathbf{0}, \mathbf{K}(\latent, \latent) \kronecker \mathbf{K}_{\text{data-meta}}(\metadata, \metadata) + \sigma^2\identity),    
\]

where $\metadata \in \reals^{D \times F}$ is the matrix of meta-features about the datasets. Inference in this models requires inversion of a covariance matrix of size $ND \times ND$, which can quickly become untractable unless computational techniques for the efficient inversion of matrix-variate normal distributions are used \citep{stegle2011efficient}.

Examples of workflow metadata could be information about which components or parameters are used in each workflow. This information can then be incorporated in the model again using the covariance function
\[
p(\data \given \latent, \btheta, \sigma, \metadata) = \mathcal{N}(\mathbf{0}, \mathbf{K}(\latent, \latent) +  \mathbf{K}_{\text{workflow-meta}}(\metadata, \metadata) + \sigma^2\identity),    
\]

where in this case $\metadata \in \reals^{N \times F}$ is the matrix of meta-features about the workflows. Inference in this model is as efficient as in the model described in section \ref{sec:main}  because we can still exploit the sparsity in $\data$ to marginalize out missing values. 

\subsection{Automated ensembling}
After training the model, we can use it to visualize the latent space where the models are embedded. Figure \ref{fig:embedding} shows the embedding of $5,000$ models in the OpenML datasets described below. Each dot is a model and the color corresponds to the AUC in one of the datasets (Figure \ref{fig:embedding_different} shows the same plot for multiple different datasets). Given a new dataset, we can not only predict the performance of a workflow that we have already observed (i.e. one of the points), but also the performance of models we have never seen, corresponding to computing predictions falling in the gray part of the plot. Using vector algebra, we can then find which combination of models will allow us to reach that particular point of the latent space. 

\subsection{Vector performance measures}
The generation of autoML training data yields multiple performance measures per dataset, e.g., accuracy, AUC, etc.
Inclusion of vector outputs in the GPLVM may improve inference for the pipeline latent embedding.
A computationally attractive algorithm is required here.
